QDOT: Quantized Dot Product Kernel for Approximate High-Performance Computing

Approximate computing techniques have been successful in reducing computation and power costs in several domains. However, error sensitive applications in high-performance computing are unable to benefit from existing approximate computing strategies that are not developed with guaranteed error bounds. While approximate computing techniques can be developed for individual high-performance computing applications by domain specialists, this often requires additional theoretical analysis and potentially extensive software modification. Hence, the development of low-level error-bounded approximate computing strategies that can be introduced into any high-performance computing application without requiring additional analysis or significant software alterations is desirable. In this paper, we provide a contribution in this direction by proposing a general framework for designing error-bounded approximate computing strategies and apply it to the dot product kernel to develop qdot -- an error-bounded approximate dot product kernel. Following the introduction of qdot, we perform a theoretical analysis that yields a deterministic bound on the relative approximation error introduced by qdot. Empirical tests are performed to illustrate the tightness of the derived error bound and to demonstrate the effectiveness of qdot on a synthetic dataset, as well as two scientific benchmarks -- Conjugate Gradient (CG) and the Power method. In particular, using qdot for the dot products in CG can result in a majority of components being perforated or quantized to half precision without increasing the iteration count required for convergence to the same solution as CG using a double precision dot product.

==> Makefile <==
SRC=zfp_stability_paper

all: 
	pdflatex "\def\isFinal{false}\def\isLBL{false} \input{$(SRC)}"
	bibtex $(SRC) 
	pdflatex "\def\isFinal{false}\def\isLBL{false} \input{$(SRC)}"
	pdflatex "\def\isFinal{false}\def\isLBL{false} \input{$(SRC)}"

final:
	pdflatex -jobname=$(SRC)_final "\def\isFinal{true}\def\isLBL{false} \input{$(SRC)}"
	bibtex $(SRC)_final
	pdflatex -jobname=$(SRC)_final "\def\isFinal{true}\def\isLBL{false} \input{$(SRC)}"
	pdflatex -jobname=$(SRC)_final "\def\isFinal{true}\def\isLBL{false} \input{$(SRC)}"

lbl:
	pdflatex -jobname=$(SRC)_lbl "\def\isFinal{true}\def\isLBL{true} \input{$(SRC)}"
	bibtex $(SRC)_lbl
	pdflatex -jobname=$(SRC)_lbl "\def\isFinal{true}\def\isLBL{true} \input{$(SRC)}"
	pdflatex -jobname=$(SRC)_lbl "\def\isFinal{true}\def\isLBL{true} \input{$(SRC)}"

view:
	make all
	acroread ${SRC}.pdf

clean:
	rm -rf *dvi *idx *log *toc *lof *lot *bbl *aux *blg *out *~ ${SRC}*.pdf



==> infocollection.tex <==
\section{qdot Implementation Details} \label{sec:qdot-implementation}
\textcolor{red}{(This section will now just contain some specific implementation details (like use of exact binning, cublas functions, etc.) and reasoning for our choice of methods for the implementation.)} We now provide details on our implementation of qdot together with runtime and memory analysis to motivate choices behind our design. To ensure our discussion is focused, we only provide analysis for the techniques used in our implementation but we note that other approaches for binning and sorting are analyzed and discussed in detail in Appendix~\ref{sec:appendixa}.

\subsection{Exponent-based Binning: Information Collection Phase} \label{sec:q-dot-pre-init}
We now turn our attention to discussing different binning strategies and considering the overhead cost associated with each strategy. In particular, all of the strategies we discuss can summarized at a high level in three steps:
\begin{enumerate}
    \item \textbf{Exponent Preprocessing.} Compute componentwise sum of exponent for each component of $\bm{x}$ and $\bm{y}$. Note that some methods may requiring keeping track of the maximum and minimum exponent value.
    \item \textbf{Initialize Index Bins of Preprocessed Exponents.} This step may involve sorting the preprocessed exponent array.
    \item \textbf{Modify Bin Score to Reduce Computation Cost and Error.} This step is the notable difference between the different binning strategies. The goal here is to tune the bin size and precision parameters in a manner that reduces the computation cost while achieving the desired error bound. Based on the formula for the bin score in (E.3), the only tunable bin parameters independent of the inputs $\bm{x}$ and $\bm{y}$ are the maximum exponent and bin size.
\end{enumerate}
To supplement the theoretical presentation and analysis of this approach we provide a graphic that illustrates the exponent-based binning preprocessing pipeline. Step 1 is the same for all techniques. Step 2 is similar across most techniques. The process of determining the bins in Step 3 is different for each technique. 

\begin{center}
\resizebox{0.95\textwidth}{!}{%
\begin{tikzpicture}[even odd rule,rounded corners=2pt,x=4pt,y=4pt]
% Step boxes
    % Step 1: Exponent preprocessing box
    \filldraw[thick,fill=red!20]
        (-10.5,-10) rectangle (-6,-33) node[pos=.5,rotate=90] {\bfseries Exp. Preproc.} ;
    \filldraw[thick,fill=red!5] 
        (-5.5,-10) rectangle (111,-33) ;
    % Step 2: Bin initialization box
    \filldraw[thick,fill=green!20]
        (-10.5,-33.5) rectangle (-6,-50.1) node[pos=.5,rotate=90] {\bfseries Bin Init.} ;
    \filldraw[thick,fill=green!5] 
        (-5.5,-33.5) rectangle (111,-50.1) ;
    % Step 3: Bin Score
    \filldraw[thick,fill=orange!20]
        (-10.5,-50.6) rectangle (-6,-86) node[pos=.5,rotate=90] {\bfseries Bin Scoring} ;
    \filldraw[thick,fill=orange!5] 
        (-5.5,-50.6) rectangle (111,-86) ;
% x and y vectors
    % x and y boxes
    %\filldraw[fill=red!30] 
    %    (0,0) rectangle (40,3) 
    %    (70,0) rectangle (110,3) ;
    % nodes for center of x and y
    %\node (x) at (20, 0) {};
    %\node (y) at (90, 0) {};
    % x and y labels
    %\node at (-3,1.5) {$\bm{x}$};
    %\node at (67,1.5) {$\bm{y}$};
% x_e and y_e vectors
    % x_e and y_e boxes
    \filldraw[fill=red!30] 
        (0,-15) rectangle (40,-12) 
        (70,-15) rectangle (110,-12) ;
    % nodes for top of x_e and y_e
    \node (x_e_top) at (20, -12) {};
    \node (y_e_top) at (90, -12) {};
    % nodes for bottom of x_e and y_e
    \node (x_e) at (19, -16) {};
    \node (y_e) at (91, -16) {};
    % x and y labels
    \node at (-3,-13.5) {$\bm{x}$};
    \node at (67,-13.5) {$\bm{y}$};
% Addition for x_e and y_e
    % node for combining x_e and y_e
        \node (x_plus_y) at (55, -20) {};
    % nodes for left and right of x_e + y_e
        \node (x_plus_y_left) at (50, -20) {} ;
        \node (x_plus_y_right) at (60, -20) {} ;
% e vector
    % e box
    \filldraw[fill=red!30] 
        (30,-31) rectangle (80,-28) ;
    % nodes for top of e
    \node (e_top) at (55, -28) {};
    % nodes for bottom of e
    \node (e) at (55, -31) {};
    % e label
    \node at (27,-29.5) {$\bm{e}$};
    % e entries
    \node at (33,-29.7) {$e_1$} ;
    \node at (44,-29.7) {$\cdots$} ;
    \node at (55,-29.7) {$e_j$} ;
    \node at (66,-29.7) {$\cdots$} ;
    \node at (77,-29.7) {$e_n$} ;
    % e vector lines
    \draw (36,-31) -- (36,-28);
    \draw (52,-31) -- (52,-28);
    \draw (58,-31) -- (58,-28);
    \draw (74,-31) -- (74,-28);
% e_sorted vector
    % e_sorted box
    \filldraw[fill=green!30] 
        (30,-48.1) rectangle (80,-45.1) ;
    % node for top of e_sorted
    \node (e_sorted_top) at (55, -45.1) {};
    % nodes for bottom of e_sorted
    \node (e_sorted) at (55, -48.1) {};
    \node (e_s1) at (33, -48.5) {};
    \node (e_s12) at (37, -48.9) {};
    \node (e_s13) at (42, -49) {};
    \node (e_sj) at (55, -48.3) {};
    \node (e_sj1) at (49, -48.9) {};
    \node (e_sj3) at (61, -48.9) {};
    \node (e_sn) at (77, -48.5) {};
    \node (e_sn1) at (68, -49) {};
    \node (e_sn2) at (73, -48.9) {};
    % e_sorted label
    \node at (26,-46.6) {$\bm{e}_{init}$};
    % e_sorted entries
    \node at (33,-46.8) {$e_{i_1}$} ;
    \node at (44,-46.8) {$\cdots$} ;
    \node at (55,-46.8) {$e_{i_j}$} ;
    \node at (66,-46.8) {$\cdots$} ;
    \node at (77,-46.8) {$e_{i_n}$} ;
    % e_sorted vector lines
    \draw (36,-48.1) -- (36,-45.1);
    \draw (52,-48.1) -- (52,-45.1);
    \draw (58,-48.1) -- (58,-45.1);
    \draw (74,-48.1) -- (74,-45.1);
% Exponent bins
    % bin boxes
    \filldraw[fill=blue!30] 
        (5,-65) rectangle (15,-62) 
        (50,-65) rectangle (60,-62)
        (95,-65) rectangle (105,-62) ;
    % ellipses nodes
    \node (bdots1) at (30, -63.5) {\Huge $\cdots$};
    \node (bdots2) at (75, -63.5) {\Huge $\cdots$};
    % nodes for top of bins
    \node (b1_top) at (10, -61.5) {};
    \node (bj_top) at (55, -62.5) {};
    \node (bk_top) at (100, -61.5) {};
    % nodes for bottom of bins
    \node (b1_bottom) at (10, -65) {};
    \node (bj_bottom) at (55, -65) {};
    \node (bk_bottom) at (100, -65) {};
    \node (bdots1_bottom) at (30, -65) {};
    \node (bdots2_bottom) at (75, -65) {};
    % bin labels
    \node (b1) at (0, -63.5) {$B_{\ell_1, u_1}$};
    \node (bj) at (45, -63.5) {$B_{\ell_j, u_j}$};
    \node (bk) at (90, -63.5) {$B_{\ell_k, u_k}$};
% Exponent bins with precision
    % bin boxes
    \filldraw[fill=blue!30] 
        (5,-80) rectangle (15,-77) 
        (50,-80) rectangle (60,-77)
        (95,-80) rectangle (105,-77) ;
    % ellipses nodes
    \node (pdots1) at (30, -78.5) {\Huge $\cdots$};
    \node (pdots2) at (75, -78.5) {\Huge $\cdots$};
    % nodes for top of bins
    \node (p1_top) at (10, -76.5) {};
    \node (pj_top) at (55, -76.5) {};
    \node (pk_top) at (100, -76.5) {};
    \node (pdots1_top) at (30, -76.5) {};
    \node (pdots2_top) at (75, -76.5) {};
    % bin labels
    \node (p1) at (0, -78.5) {$B_{\ell_1, u_1}$};
    \node (prec1) at (10, -83) {$half$};
    \node (pj) at (45, -78.5) {$B_{\ell_j, u_j}$};
    \node (precj) at (55, -83) {$single$};
    \node (pk) at (90, -78.5) {$B_{\ell_k, u_k}$};
    \node (precj) at (100, -83) {$quad$};
% arrows connecting arrays
    % x -> x_e and y -> y_e
    %\draw[->, thick] (x) -- (x_e_top) node[midway,left] {$\texttt{frexp}$} ;
    %\draw[->, thick] (y) -- (y_e_top) node[midway,left] {$\texttt{frexp}$} ;
    % x , y -> x_e + y_e
    \draw[-, thick] (x_e) -- (x_plus_y_left) ;
    \draw[-, thick] (y_e) -- (x_plus_y_right) ;
    % x_e + y_e -> e
    \draw[->, thick] (x_plus_y) -- (e_top) ;
    \node[fill=white] (x_plus_y_text) at (55, -20) {$\texttt{frexp}(\bm{x}) + \texttt{frexp}(\bm{y})$} ;
    % e -> e_sorted
    \draw[->, thick] (e) -- (e_sorted_top) node[midway,fill=white] {Unsorted or sorted bin initialization} ;
    % e_sorted -> exponent bins
    \coordinate (merge1) at (28, -54);
    \draw[-,thick] (e_s1) to (merge1) ;
    \draw[-,thick] (e_s12) to (merge1) ;
    \draw[-,thick] (e_s13) to (merge1) ;
    \draw[->, thick] (merge1) -- (b1_top) node[midway,fill=white] {$\{ i : \ell_1 < e_i \leq u_1 \}$} ;
    \coordinate (mergej) at (55, -53);
    \draw[-,thick] (e_sj) to (mergej) ;
    \draw[-,thick] (e_sj1) to (mergej) ;
    \draw[-,thick] (e_sj3) to (mergej) ;
    \draw[->, thick] (mergej) -- (bj_top) node[midway,fill=white] {$\{ i : \ell_j < e_i \leq u_j \}$} ;
    \coordinate (mergen) at (82, -54);
    \draw[-,thick] (e_sn) to (mergen) ;
    \draw[-,thick] (e_sn1) to (mergen) ;
    \draw[-,thick] (e_sn2) to (mergen) ;
    \draw[->, thick] (mergen) -- (bk_top) node[midway,fill=white] {$\{ i : \ell_n < e_i \leq u_n \}$} ;
    % exponent bins -> precision bins
    \draw[->, thick] (b1_bottom) -- (p1_top) ;
    \draw[->, thick] (bdots1_bottom) -- (pdots1_top) ;
    \draw[->, thick] (bj_bottom) -- (pj_top) ;
    \draw[->, thick] (bdots2_bottom) -- (pdots2_top) ;
    \draw[->, thick] (bk_bottom) -- (pk_top) ;
    \fill[fill=white] 
        (5,-69) rectangle (105,-73) node[pos=.5] {Use (\ref{eq:precision-def}) to determine quantization level} ;
\end{tikzpicture}}
\end{center}

\iffalse %%%%%%%%%%%%%%%%%%%%%%
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[even odd rule,rounded corners=2pt,x=4pt,y=4pt]
% Step boxes
    % Step 1: Exponent preprocessing box
    \filldraw[thick,fill=red!20]
        (-10.5,-10) rectangle (-6,-33) node[pos=.5,rotate=90] {\bfseries Step 1} ;
    \filldraw[thick,fill=red!5] 
        (-5.5,-10) rectangle (111,-33) ;
    % Step 2: Bin initialization box
    \filldraw[thick,fill=green!20]
        (-10.5,-33.5) rectangle (-6,-50.1) node[pos=.5,rotate=90] {\bfseries Step 2} ;
    \filldraw[thick,fill=green!5] 
        (-5.5,-33.5) rectangle (111,-50.1) ;
    % Step 3: Bin Score
    \filldraw[thick,fill=orange!20]
        (-10.5,-50.6) rectangle (-6,-86) node[pos=.5,rotate=90] {\bfseries Step 3} ;
    \filldraw[thick,fill=orange!5] 
        (-5.5,-50.6) rectangle (111,-86) ;
% x and y vectors
    % x and y boxes
    %\filldraw[fill=red!30] 
    %    (0,0) rectangle (40,3) 
    %    (70,0) rectangle (110,3) ;
    % nodes for center of x and y
    %\node (x) at (20, 0) {};
    %\node (y) at (90, 0) {};
    % x and y labels
    %\node at (-3,1.5) {$\bm{x}$};
    %\node at (67,1.5) {$\bm{y}$};
% x_e and y_e vectors
    % x_e and y_e boxes
    \filldraw[fill=red!30] 
        (0,-15) rectangle (40,-12) 
        (70,-15) rectangle (110,-12) ;
    % nodes for top of x_e and y_e
    \node (x_e_top) at (20, -12) {};
    \node (y_e_top) at (90, -12) {};
    % nodes for bottom of x_e and y_e
    \node (x_e) at (19, -16) {};
    \node (y_e) at (91, -16) {};
    % x and y labels
    \node at (-3,-13.5) {$\bm{x}$};
    \node at (67,-13.5) {$\bm{y}$};
% Addition for x_e and y_e
    % node for combining x_e and y_e
        \node (x_plus_y) at (55, -20) {};
    % nodes for left and right of x_e + y_e
        \node (x_plus_y_left) at (50, -20) {} ;
        \node (x_plus_y_right) at (60, -20) {} ;
% e vector
    % e box
    \filldraw[fill=red!30] 
        (30,-31) rectangle (80,-28) ;
    % nodes for top of e
    \node (e_top) at (55, -28) {};
    % nodes for bottom of e
    \node (e) at (55, -31) {};
    % e label
    \node at (27,-29.5) {$\bm{e}$};
    % e entries
    \node at (33,-29.7) {$e_1$} ;
    \node at (44,-29.7) {$\cdots$} ;
    \node at (55,-29.7) {$e_j$} ;
    \node at (66,-29.7) {$\cdots$} ;
    \node at (77,-29.7) {$e_n$} ;
    % e vector lines
    \draw (36,-31) -- (36,-28);
    \draw (52,-31) -- (52,-28);
    \draw (58,-31) -- (58,-28);
    \draw (74,-31) -- (74,-28);
% e_sorted vector
    % e_sorted box
    \filldraw[fill=green!30] 
        (30,-48.1) rectangle (80,-45.1) ;
    % node for top of e_sorted
    \node (e_sorted_top) at (55, -45.1) {};
    % nodes for bottom of e_sorted
    \node (e_sorted) at (55, -48.1) {};
    \node (e_s1) at (33, -48.5) {};
    \node (e_s12) at (37, -48.9) {};
    \node (e_s13) at (42, -49) {};
    \node (e_sj) at (55, -48.3) {};
    \node (e_sj1) at (49, -48.9) {};
    \node (e_sj3) at (61, -48.9) {};
    \node (e_sn) at (77, -48.5) {};
    \node (e_sn1) at (68, -49) {};
    \node (e_sn2) at (73, -48.9) {};
    % e_sorted label
    \node at (26,-46.6) {$\bm{e}_{init}$};
    % e_sorted entries
    \node at (33,-46.8) {$e_{i_1}$} ;
    \node at (44,-46.8) {$\cdots$} ;
    \node at (55,-46.8) {$e_{i_j}$} ;
    \node at (66,-46.8) {$\cdots$} ;
    \node at (77,-46.8) {$e_{i_n}$} ;
    % e_sorted vector lines
    \draw (36,-48.1) -- (36,-45.1);
    \draw (52,-48.1) -- (52,-45.1);
    \draw (58,-48.1) -- (58,-45.1);
    \draw (74,-48.1) -- (74,-45.1);
% Exponent bins
    % bin boxes
    \filldraw[fill=blue!30] 
        (5,-65) rectangle (15,-62) 
        (50,-65) rectangle (60,-62)
        (95,-65) rectangle (105,-62) ;
    % ellipses nodes
    \node (bdots1) at (30, -63.5) {\Huge $\cdots$};
    \node (bdots2) at (75, -63.5) {\Huge $\cdots$};
    % nodes for top of bins
    \node (b1_top) at (10, -61.5) {};
    \node (bj_top) at (55, -62.5) {};
    \node (bk_top) at (100, -61.5) {};
    % nodes for bottom of bins
    \node (b1_bottom) at (10, -65) {};
    \node (bj_bottom) at (55, -65) {};
    \node (bk_bottom) at (100, -65) {};
    \node (bdots11_bottom) at (27, -65) {};
    \node (bdots12_bottom) at (33, -65) {};
    \node (bdots21_bottom) at (72, -65) {};
    \node (bdots22_bottom) at (78, -65) {};
    % bin labels
    \node (b1) at (0, -63.5) {$B_{\ell_1, u_1}$};
    \node (bj) at (45, -63.5) {$B_{\ell_j, u_j}$};
    \node (bk) at (90, -63.5) {$B_{\ell_k, u_k}$};
% Precision bins
    % precision boxes
    \filldraw[fill=orange!30] 
        (3,-80) rectangle (19,-77) 
        (25,-80) rectangle (41,-77) 
        (47,-80) rectangle (63,-77) 
        (69,-80) rectangle (85,-77) 
        (91,-80) rectangle (107,-77)  ;
    % nodes for top of precision bins
    \node (perf_top) at (11, -77) {};
    \node (half_top) at (33, -77) {};
    \node (single_top) at (55, -77) {};
    \node (double_top) at (77, -77) {};
    \node (quad_top) at (99, -77) {};
    % precision bin labels
    \node (p_p) at (11, -83) {$P_{perforate}$};
    \node (p_h) at (33, -83) {$P_{half}$};
    \node (p_s) at (55, -83) {$P_{single}$};
    \node (p_d) at (77, -83) {$P_{double}$};
    \node (p_q) at (99, -83) {$P_{quad}$};
% arrows connecting arrays
    % x -> x_e and y -> y_e
    %\draw[->, thick] (x) -- (x_e_top) node[midway,left] {$\texttt{frexp}$} ;
    %\draw[->, thick] (y) -- (y_e_top) node[midway,left] {$\texttt{frexp}$} ;
    % x , y -> x_e + y_e
    \draw[-, thick] (x_e) -- (x_plus_y_left) ;
    \draw[-, thick] (y_e) -- (x_plus_y_right) ;
    % x_e + y_e -> e
    \draw[->, thick] (x_plus_y) -- (e_top) ;
    \node[fill=white] (x_plus_y_text) at (55, -20) {$\texttt{frexp}(\bm{x}) + \texttt{frexp}(\bm{y})$} ;
    % e -> e_sorted
    \draw[->, thick] (e) -- (e_sorted_top) node[midway,fill=white] {Unsorted or sorted bin initialization} ;
    % e_sorted -> exponent bins
    \coordinate (merge1) at (28, -54);
    \draw[-,thick] (e_s1) to (merge1) ;
    \draw[-,thick] (e_s12) to (merge1) ;
    \draw[-,thick] (e_s13) to (merge1) ;
    \draw[->, thick] (merge1) -- (b1_top) node[midway,fill=white] {$\{ i : \ell_1 < e_i \leq u_1 \}$} ;
    \coordinate (mergej) at (55, -53);
    \draw[-,thick] (e_sj) to (mergej) ;
    \draw[-,thick] (e_sj1) to (mergej) ;
    \draw[-,thick] (e_sj3) to (mergej) ;
    \draw[->, thick] (mergej) -- (bj_top) node[midway,fill=white] {$\{ i : \ell_j < e_i \leq u_j \}$} ;
    \coordinate (mergen) at (82, -54);
    \draw[-,thick] (e_sn) to (mergen) ;
    \draw[-,thick] (e_sn1) to (mergen) ;
    \draw[-,thick] (e_sn2) to (mergen) ;
    \draw[->, thick] (mergen) -- (bk_top) node[midway,fill=white] {$\{ i : \ell_n < e_i \leq u_n \}$} ;
    % exponent bins -> precision bins
    \draw[->, thick] (b1_bottom) -- (perf_top) ;
    \draw[->, thick] (bdots11_bottom) -- (half_top) ;
    \draw[->, thick] (bdots12_bottom) -- (single_top) ;
    \draw[->, thick] (bj_bottom) -- (single_top) ;
    \draw[->, thick] (bdots21_bottom) -- (double_top) ;
    \draw[->, thick] (bdots22_bottom) -- (quad_top) ;
    \draw[->, thick] (bk_bottom) -- (quad_top) ;
    \fill[fill=white] 
        (5,-69) rectangle (105,-73) node[pos=.5] {Use rules in (E.4) to determine quantization level} ;
\end{tikzpicture}}
\end{center}
\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%

As each of these strategies require binning based on exponent values, the first step will always require preprocessing the exponent values. The cost associated with this preprocessing step and its analysis is included here so that it does not need to be repeated for each method. Additionally, since many of the bin initialization steps require sorting, we discuss sorting analysis and costs here so they do not have to be repeated during each strategy. The following section will focus on discussing different strategies and their associated costs. 


\iffalse
\subsection{Exponent Preprocessing Step} \label{sec:q-dot-preprocess}

We now provide pseudocode for the exponent preprocessing step, in Algorithm~\ref{alg:exp-preprocessing}, and determine the associated cost, in Theorem~\ref{thm:exp-preprocessing}.
\begin{center}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE{\textit{Inputs}: $\bm{x}, \bm{y} \in \mathbb{R}^n$.}
\STATE{\textit{Initialize Variables}: short int $x_e$, $y_e$, $m_{x,y}$, $M_{x,y}$, $e[n]$ ; Set $m_{x,y} = \infty$ and $M_{x,y} = -\infty$.}
\FOR{$i=1$ to $n$}
    \STATE{\textit{Extract Exponents}: frexp$(x[i], \& x_e)$; frexp$(y[i], \& y_e)$;} 
    \STATE{\textit{Add Exponents}: $e[i] = x_e + y_e$;}
    \STATE{\textit{Update Minimum and Maximum Exponent}:} 
    \IF{$(e[i] < m_{x,y})$}
        \STATE{$m_{x,y} = e[i]$ ;}
    \ELSIF{$(e[i] > M_{x,y})$} 
        \STATE{$M_{x,y} = e[i]$ ;}
    \ENDIF
\ENDFOR
\STATE{\textit{Return} $e$, $m_{x,y}$, and $M_{x,y}$.}
\end{algorithmic}
\caption{\texttt{EP} - Exponent Preprocessing}
\label{alg:exp-preprocessing}
\end{algorithm}
\end{center}

\begin{theorem} \label{thm:exp-preprocessing}
\texttt{EP}, Algorithm~\ref{alg:exp-preprocessing}, has a worst-case runtime of $O(n)$ and a memory overhead of $O(n)$.
\end{theorem}
\begin{proof}
We derive the runtime cost by considering each operation required by Algorithm~\ref{alg:exp-preprocessing}. The following operations are required for each index $i \in [n]$:
\begin{itemize}
    \item Extracting the exponent for each component of $\bm{x}$ and $\bm{y}$: 2 exponent accesses (\texttt{frexp} function)
    \item Adding the exponent values: 1 integer addition operation
    \item Storing in key-value pairs $(e[i], i)$: Up to 2 insertion operations depending on how they are stored (e.g., array only requires one insertion operation).
\end{itemize}
For methods that require the minimum and maximum exponent values, denoted $m_{x,y}$ and $M_{x,y}$ respectively, the following operations are also necessary:
\begin{itemize}
    \item Compare exponent $e[i]$ to the current minimum and maximum exponent values and update if necessary: Requires at most 2 compare operations and at most 1 assignment operation.
\end{itemize}
Hence, there are a total of at most $8n$ operations yielding the associated runtime of $O(n)$.

The associated memory overhead follows from the need for the array $e$ of size $n$ and 4 additional variables. 
\end{proof}

Before proceeding to the next step, we establish necessary conditions for performing an early termination after exponent preprocessing. In particular, this result indicates that we can determine if no approximation will be applied by using the values $M_{x,y}$, $m_{x,y}$, and $p_{x,y}$ .

\begin{theorem} \label{thm:early-termination}
Let $\bm{x}, \bm{y} \in \mathbb{R}^n$ and let $\hat{p}_{x,y}$ denote the number of mantissa bits for the level of precision directly below $p_{x,y}$. If $M_{x,y} - m_{x,y} \leq p_{x,y} - \hat{p}_{x,y}$ then the level of precision specified for all bins will be $p_{x,y}$ based on the rules in (E.4).
\end{theorem}
\begin{proof}
Suppose $M_{x,y} - m_{x,y} \leq p_{x,y} - \hat{p}_{x,y}$. Then
\begin{align}
    \hat{p}_{x,y} 
    &\leq p_{x,y} - M_{x,y} + m_{x,y}. \label{eq:early-termination.1}
\end{align}
Combining (\ref{def:bin-score}) together with the fact that $b_k \geq 0$ and $u_k \geq m_{x,y}$, it now follows that
\begin{align}
    \hat{p}_{x,y} 
    &\leq p_{x,y} - M_{x,y} + m_{x,y}
    \leq p_{x,y} - M_{x,y} + b_k + u_k 
    = \beta_k, \label{eq:early-termination.2}
\end{align}
for all $k$. As $\hat{p}_{x,y}$ is the level of precision directly below $p_{x,y}$, the rules in (E.4) yield that the precision of every bin will be $p_{x,y}$.
\end{proof}


\subsection{Sorted Exponent Bin Initialization Step} \label{sec:q-dot-initialize}
We now provide pseudocode for the sorted exponent bin initialization step, in Algorithm~\ref{alg:sort-bin-init}, and determine the associated cost, in Theorem~\ref{thm:sort-bin-init}.

\begin{center}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE{\textit{Inputs}: Preprocessed Exponent Array $e \in \mathbb{Z}^n$, min and max exponents $m_{x,y}$ and $M_{x,y}$.}
\STATE{\textit{Identify and Use Faster Sorting Method}:} 
\IF{$M_{x,y} - m_{x,y} + 1 \leq n \log_2 (n/2)$}
    \STATE{$e_{sorted}, e_{count} \gets \texttt{counting\_sort}(e)$}
\ELSE
    \STATE{$e_{sorted} \gets \texttt{merge\_sort}(e)$}
    \STATE{Count number of appearances of each exponent in $e_{sorted}$ and store in array $e_{count}$}
\ENDIF
\STATE{\textit{Return Arrays} $e_{sorted}$ and $e_{count}$.}
\end{algorithmic}
\caption{\texttt{SBI} - Sorted (Exponent) Bin Initialization}
\label{alg:sort-bin-init}
\end{algorithm}
\end{center}

Before proving the worst-case runtime and memory overhead for Algorithm~\ref{alg:sort-bin-init}, we outline specific details for using counting sort and merge sort in Algorithm~\ref{alg:sort-bin-init}.

\begin{itemize}
    \item \textbf{Counting Sort}:
    \begin{itemize}
        \item A single use of a standard counting sort algorithm can be used to compute two arrays:
        \begin{enumerate}
            \item[(1)] $e_{sorted}$: Array of length $n$ containing indices $i$ ordered such that $e[i] \leq e[i+1]$, for $i \in [n-1]$.
            \item[(2)] $e_{count}$: Array of length $M_{x,y} - m_{x,y} + 1$ whose $i$th component is the number of instances exponent $m_{x,y} + i$ appears in array $e$
        \end{enumerate}
        \item Achieving (1) might require sorting key-value pairs $(e[i], i)$ on the keys then writing new array with just values (indices).
        \item Using $e_{count}$ and $e_{sorted}$, the information required to compute the bin score and dot product for an exact bin of the form $B_{u_k - 1, u_k} (\bm{x}, \bm{y})$ can be computed as
        \begin{align}
            B_{u_k - 1, u_k} (\bm{x}, \bm{y}) 
            &= \left\{ e_{sorted}[s_k], \ldots, e_{sorted}[s_{k+1} - 1] \right\}, \nonumber \\
            u_k &= m_{x,y} + k, \label{eq:counting-sort-bins} \\
            |B_{u_k - 1, u_k} (\bm{x}, \bm{y})| &= e_{count}[k], \nonumber
        \end{align}
        where $s_k := \sum_{i=0}^k |B_{u_k - 1, u_k} (\bm{x}, \bm{y})|$.
        \item \textit{Remark: Counting Sort Post-processing.} While not necessary, note that the output from counting sort could be processed to remove the entries where $b_k = 0$. This post-processing would take $O(n_{x,y} + M_{x,y} - m_{x,y} + 1)$ time as it would require a second pass over the sorted data. 
    \end{itemize}
    \item \textbf{Merge Sort}:
    \begin{itemize}
        \item A single use of a merge sort algorithm on an array/vector of pairs $(e[i], i)$ can be used to compute the following array:
        \begin{enumerate}
            \item[(1)] $e_{sorted}$: Array of length $n$ containing pairs $(e[i], i)$ ordered such that $e[i] \leq e[i+1]$, for $i \in [n-1]$.
        \end{enumerate}
        \item Following the sorting process an array with the frequency of each exponent can be determined by making a single pass over the keys of the $e_{sorted}$ array. This array is described below: 
        \begin{enumerate}
            \item[(2)] $e_{count}$: Array of length at most $n$ whose $i$th component is the frequency of the $i$th largest value in array $e$
        \end{enumerate}
        \item Using $e_{count}$ and $e_{sorted}$, the information required to compute the bin score and dot product for an exact bin of the form $B_{u_k - 1, u_k} (\bm{x}, \bm{y})$ can be computed as
        \begin{align}
            B_{u_k - 1, u_k} (\bm{x}, \bm{y}) 
            &= \left\{ e_{sorted}[s_k][1], \ldots, e_{sorted}[s_{k+1} - 1][1] \right\}, \nonumber \\
            u_k &= e_{sorted}[s_k][0], \label{eq:merge-sort-bins} \\
            |B_{u_k - 1, u_k} (\bm{x}, \bm{y})| &= e_{count}[k], \nonumber
        \end{align}
        where $s_k := \sum_{i=0}^k |B_{u_k - 1, u_k} (\bm{x}, \bm{y})|$.
    \end{itemize}
\end{itemize}
%Note that $e_{sorted}$ is an array of length $n$ of key-value pairs $(e[i], i)$ sorted by keys (exponent value). When counting sort is used $e_{count}$ is an array generated during the sorting process of length $M_{x,y} - m_{x,y} + 1$ in which the $k$th entry corresponds to the number of times the exponent $m_{x,y} + k$ appears in the array $e$. When merge sort is used, $e_{count}$ is an array generated after the sorting process whose length is the number of distinct exponents in $e$ and the $k$th entry of $e_{count}$ corresponds to the number of times the $k$th largest exponent appearing in the array $e$.

We now prove the worst-case runtime and memory overhead associated with Algorithm~\ref{alg:sort-bin-init}.

\begin{theorem} \label{thm:sort-bin-init}
\texttt{SBI}, Algorithm~\ref{alg:sort-bin-init}, has a worst-case runtime of $O(\min \{ n + M_{x,y} - m_{x,y}, n\log_2 n \})$ and memory overhead of $O(n + M_{x,y} - m_{x,y})$. 
\end{theorem}
\begin{proof}
We derive this cost by considering each operation required by Algorithm~\ref{alg:sort-bin-init}. %Since we are sorting integer values, we are not limited to comparison based sorting methods. With this in mind, we can compare the associated known costs of each sorting method directly before sorting to choose the method with a lower cost. 
First, note that counting sort has a worst-case cost of $O(n + k)$, where $n$ is the number of elements being sorted and $k$ is the number of distinct values that the $n$ elements can have. From Algorithm~\ref{alg:exp-preprocessing}, we find that the array $e$ has at most $M_{x,y} - m_{x,y} + 1$ distinct values. Hence, the worst-case cost for using counting sort in Algorithm~\ref{alg:sort-bin-init} is $O(n + M_{x,y} - m_{x,y} + 1)$. On the other hand, merge sort has a worst-case cost of $O(n \log_2 n)$ and computing $e_{count}$ after merge sort hasa worst-case scenario cost of $O(n)$. Hence, the cost associated with using merge sort in Algorithm~\ref{alg:sort-bin-init} is $O(n \log_2 n)$. 

The heuristic for choosing which sorting algorithm will be (approximately) faster can now be derived by observing that
\begin{align*}
    n + M_{x,y} - m_{x,y} + 1 \leq n \log_2 n 
    \quad \Longleftrightarrow \quad
    M_{x,y} - m_{x,y} + 1 \leq n (\log_2 n - 1) = n \log_2 (n/2),
\end{align*}
for $n \geq 2$. Based on this criterion, the following rules for choosing a sorting method will result in a worst-case cost of $O(\min \{ n + M_{x,y} - m_{x,y}, n\log_2 n \})$:
\begin{itemize}
    \item \textit{When to Use Counting Sort}: If $M_{x,y} - m_{x,y} + 1 \leq n \log_2 (n/2)$, where $m_{x,y}$ and $M_{x,y}$ are the minimum and maximum exponent values from the preprocessing step, then use counting sort which has an associated cost of $O(n + M_{x,y} - m_{x,y} + 1)$.
    \item \textit{When to Use Merge Sort}: If $M_{x,y} - m_{x,y} + 1 > n \log_2 (n/2)$ then use merge sort which has an associated cost of $O(n \log_2 n)$.
\end{itemize}
As Algorithm~\ref{alg:sort-bin-init} uses these rules to choose a sorting method, it follows that Algorithm~\ref{alg:sort-bin-init} has a worst-case cost of $O(\min \{ n + M_{x,y} - m_{x,y}, n\log_2 n \})$.

We now consider the memory overhead. If counting sort is used, the memory overhead of $O(n + M_{x,y} - m_{x,y})$ follows from standard counting sort memory complexity. If merge sort is used the memory overhead for sorting is $O(n)$. After merge sort, the array $e_{count}$ is created requiring $O(M_{x,y} - m_{x,y})$ space. Hence, the total memory overhead when merge sort is used is $O(n + M_{x,y} - m_{x,y})$. Thus, when either sorting algorithm is used the memory overhead is $O(n + M_{x,y} - m_{x,y})$.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Another note of interest is on the observed runtime of Algorithm~\ref{alg:sort-bin-init} for increasing values of $n$. We summarize this observation in the following theorem.

\begin{theorem}
For $n$ sufficiently large, $n \geq 10^4$ for IEEE Double and $n \geq 10^5$ for IEEE Quad, the worst-case runtime for Algorithm~\ref{alg:sort-bin-init} will be $O(n)$.
\end{theorem}
\begin{proof}
From Theorems~\ref{thm:double-complexity} and \ref{thm:quad-complexity}, for counting sort will be used for  As $M_{x,y} - m_{x,y} + 1$ is bounded above independent of $n$ it follows that $n + M_{x,y} - m_{x,y} + 1 \approx n$ for sufficiently large $n$ which implies that \emph{Counting Sort} will run in $O(n)$ time.
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There are two key takeaways from this analysis for \emph{IEEE Double Precision} and \emph{IEEE Quad Precision} vectors:
\begin{enumerate}
    \item \textit{Counting sort will be used for most applications}: As we expect to make up the front end costs on the back end by reduced computation costs, good candidate vectors for this approximate dot product kernel should be on the order of at least $10^2$ or $10^3$. In instances where $n$ is on the order of at least $10^2$ or $10^3$, the worst-case analysis implies that counting sort will be selected over merge sort.
    \item \textit{Counting sort will likely run in $O(n)$ time}: Based on the upper bounds for $M_{x,y} - m_{x,y} + 1$ in Theorems~\ref{thm:double-complexity} and \ref{thm:quad-complexity}, if $n \geq 10^3$ then the worst-case runtime for counting sort will be $O(n)$. It is also possible, and even likely in some applications, that the actual value of $M_{x,y} - m_{x,y} + 1$ will be much smaller than the value from the worst-case analysis as the exponents may not take up the entire range of values. Hence, it is likely that many practical applications will observe counting sort running in $O(n)$ time.
\end{enumerate}

\fi

==> old-results.tex <==
\section{Numerical Experiments}
\label{sec:results}
Experiments to demonstrate tightness of error bound.

Experiments to demonstrate use with CG.

\subsection{Tightness of Error Bound}
\label{sec:experiment-errorbound}
In the first numerical test, a 4 by 4 block was formed with absolute
values ranging from $2^{e_{min}}$ to $2^{e_{max}}$. The exponent
$e_{min}$ remains stationary while $e_{max}$ varies, depending on the
chosen exponent range. The interval $[e_{min}, e_{max}]$ was divided
into 16 evenly spaced subintervals. Each value of the block was randomly 
selected from a uniform distribution in the range
$[2^{e_{min}+(h-1)\frac{e_{max}-e_{min}}{16}},
  2^{e_{min}+h\frac{e_{max}-e_{min}}{16}}]$ with {sub}interval
$h\in \{1,\dots,16 \}$ and uniform randomly assigned sign. The block was
then randomly permuted, using the C$++$ standard library function
{\it{random\_shuffle}}, to remove any bias in the total sequency order
and then compressed and decompressed with precision, $\beta$. This
specific construction of data is designed to {mimic} the worst
possible input for ZFP for a chosen exponent range. For a given exponent
range, $\rho = e_{max}-e_{min} $, we expect the componentwise relative
error and block relative error to increase as the precision
decreases. However, {as the bound is only dependent on $\beta$,}
the block relative error bound will remain constant as the exponent
range varies. The componentwise relative error should increase as the
exponent range increases as the representable numbers in a
block-floating-point representation are dependent on the largest
exponent of the block and the value of $q$.   

For
Figures~\ref{fig:componenterror_precision_4by4}-\ref{fig:normerror_exp_4by4},
the data is represented and compressed in single-precision (32-bit IEEE
standard) with $e_{min}  = 0$, while $e_{max}$ varies with respect to
the required exponent range. Similar results {can be produced} for
any value of $e_{min}$. Figure~\ref{fig:componenterror_precision_4by4}
shows how the {componentwise relative error} (top) and block relative
error (bottom) vary with respect to the fixed precision parameter,
$\beta$, for a fixed exponent range.  For a single $\beta$, {one}
million blocks generated using the above routine were compressed and
decompressed. The blue band represents the sampled maximum and minimum
of the true componentwise relative error or block relative error, i.e.,  
\begin{align*}
\max_{i, \bx_i \neq 0} \frac{|\tilde{D}\tilde{C}\bx_i -\bx_i|} {|\bx_i|} \quad {\text{and}}  \quad \frac{\|\tilde{D}\tilde{C}\bx -\bx\|_\infty}{\|\bx\|_\infty},
\end{align*}
respectively, of all 1 million runs. The red line depicts the
theoretical bound and the dashed green line represents the asymptotic
behavior of the bound, i.e., the smallest predictive value of the
theoretical bound. For $ e_{max} - e_{min} = 0$, meaning that the
magnitude of the absolute values of the 4 by 4 block are similar, the
componentwise relative error increases as $\beta$ decreases. As the
exponent range increases, {fewer bits will be
  used to represent the smaller values in each block during Step 2 of
  ZFP, which will result in a larger relative error}. As anticipated,
{in Figure \ref{fig:componenterror_precision_4by4}} the entire plot
{shifts} toward the upper right corner as the exponent range
increases, indicating that the componentwise relative error increases
with respect to the range of compressed values. With respect to the
block relative error, the block relative error remains the same for all
$\beta$ as the exponent range varies.  

Similar trends can also be seen in Figure~\ref{fig:normerror_exp_4by4},
where the exponent range varies for a single $\beta$. In
Figure~\ref{fig:normerror_exp_4by4}, for each $\beta$, the componentwise 
relative error (top) increases as the exponent range increases while the
block relative error remains constant, as expected. As $\beta$ increases,
both the componentwise relative error and the block relative error plots
are shifted upwards, indicating an increase in error. For $\beta = 32$, there is a gap between the bound and the observed error, which corresponds to the gap in the far right of the plots in Figure~\ref{fig:componenterror_precision_4by4}, i.e., the theoretical error bound is limited to precision of the IEEE representation. It can be concluded, in
Figures~\ref{fig:componenterror_precision_4by4} and 
\ref{fig:normerror_exp_4by4}, that the theoretical bound (red) completely
bounds the maximum sampled error (blue). 

Next, we repeated this same experiment using a different machine
precision. Note that Figures~\ref{fig:2d_double_1} and
\ref{fig:2d_double_4} represent the same two-dimensional test outlined
above, but the values in the block are represented using double-precision
(64-bit IEEE standard). The same relationships can be concluded for the
double precision case.  

Finally, since the dimensionality of the block plays an important part
in ZFP, Figures~\ref{fig:1d_double_1} and \ref{fig:1d_double_4} and
Figures~\ref{fig:3d_double_1} and \ref{fig:3d_double_4} represent
results in double precision for one-dimensional and three-dimensional
blocks, respectively. Again, similar relationships can be seen as those
outlined in the two-dimensional, single-precision experiment.
%{The minimum ratio between the
%  theoretical bound and the maximum sampled error is $\approx 2.23$, for all tests so far presented.} 


%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2D, single precision  examples 
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_single0.pdf}
        \label{fig:componenterror_precision_4by4parta}
               % \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_single7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
        \label{fig:componenterror_precision_4by4partb}
    \end{subfigure}
       \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_single14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
        \label{fig:componenterror_precision_4by4partc}

    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_single0.pdf}
  %      \caption{$e_{max}- e_{min}= 0$}
                \label{fig:normerror_precision_4by4parta}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_single7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
  \label{fig:normerror_precision_4by4partb}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_single14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
  \label{fig:normerror_precision_4by4partc}
    \end{subfigure}
    \caption{2-d Example with single precision:  componentwise relative error (top) and block relative error (bottom) with respect to {the precision parameter ($\beta$) for $ e_{max}-e_{min} \in \{ 0,7,14\} $.  The blue band represents the sampled maximum and minimum error, the red line depicts the theoretical bound, and the dashed green line represents the asymptotic behavior of the theoretical bound. } }
                \label{fig:componenterror_precision_4by4}

\end{figure}

\begin{figure}
    \centering
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_2d_single12.pdf}
%\caption{$\beta = 22$}
    \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_2d_single22.pdf}
%\caption{$\beta = 27$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_2d_single32.pdf}
   %     \caption{$\beta = 32$}
    \end{subfigure}
          
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_2d_single12.pdf}
%\caption{$\beta = 22$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_2d_single22.pdf}
%\caption{$\beta = 27$}
\end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_2d_single32.pdf}
%        \caption{$\beta= 32$}
    \end{subfigure}
      \caption{2-d Example with single precision:  componentwise relative error (top) and block relative error (bottom) with respect to the difference in exponents ($e_{max}-e_{min}$) for $\beta \in \{12,22,32\}${. The blue band represents the sampled maximum and minimum error and the red line depicts the theoretical bound. }}
    \label{fig:normerror_exp_4by4}
\end{figure}
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2D, double precision  examples 
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_double0.pdf}
      %  \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
       \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_2d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}

    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_double0.pdf}
   %     \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_2d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
    \end{subfigure}
  \caption{2-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the precision parameter ($\beta$) for $ e_{max}-e_{min} \in \{0,7,14\}${. The blue band represents the sampled maximum and minimum error, the red line depicts the theoretical bound, and the dashed green line represents the asymptotic behavior of the theoretical bound. }}
    \label{fig:2d_double_1}
\end{figure}

\begin{figure}
    \centering
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_rel_2d_double32.pdf}
%    %    \caption{$\beta = 64$}
%    \end{subfigure}
%        \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_rel_2d_double48.pdf}
%%\caption{$\beta = 60$}
%    \end{subfigure}
%        \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_rel_2d_double64.pdf}
%%\caption{$\beta = 56$}
%\end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_norm_2d_double32.pdf}
% %       \caption{$\beta= 64$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_norm_2d_double48.pdf}
%%\caption{$\beta = 60$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/precision_norm_2d_double64.pdf}
%%\caption{$\beta = 56$}
%    \end{subfigure}
 \caption{2-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the difference in exponents ($e_{max}-e_{min}$) for $\beta \in \{32,48,64\}${. The blue band represents the sampled maximum and minimum error and the red line depicts the theoretical bound.}}
     \label{fig:2d_double_4}
\end{figure}

%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%1D, double precision  examples 
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_1d_double0.pdf}
     %   \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_1d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
       \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_1d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_1d_double0.pdf}
    %    \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_1d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_1d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
    \end{subfigure}
  \caption{1-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the precision parameter ($\beta$) for $ e_{max}-e_{min} \in\{ 0,7,14\}${. The blue band represents the sampled maximum and minimum error, the red line depicts the theoretical bound, and the dashed green line represents the asymptotic behavior of the theoretical bound. }}
      \label{fig:1d_double_1}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_1d_double32.pdf}
 %       \caption{$\beta = 64$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_1d_double48.pdf}
%\caption{$\beta = 60$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_1d_double64.pdf}
%\caption{$\beta = 56$}
\end{subfigure}

    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_1d_double32.pdf}
 %       \caption{$\beta= 64$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_1d_double48.pdf}
%\caption{$\beta = 60$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_1d_double64.pdf}
%\caption{$\beta = 56$}
    \end{subfigure}
 \caption{1-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the difference in exponents ($e_{max}-e_{min}$) for $\beta \in \{32,48,64\}${. The blue band represents the sampled maximum and minimum error and the red line depicts the theoretical bound. }}
    \label{fig:1d_double_4}
\end{figure}


%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%3D, double precision  examples 
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_3d_double0.pdf}
  %      \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_3d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
       \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_rel_3d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}

    \end{subfigure}

    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_3d_double0.pdf}
   %     \caption{$e_{max}- e_{min}= 0$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_3d_double7.pdf}
%\caption{$e_{max}- e_{min}= 7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/expadd_norm_3d_double14.pdf}
%\caption{$e_{max}- e_{min}= 14$}
    \end{subfigure}
  \caption{3-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the precision parameter ($\beta$) for $ e_{max}-e_{min} \in \{0,7,14\}${. The blue band represents the sampled maximum and minimum of the error, the red line depicts the theoretical bound, and the dashed green line represents the asymptotic behavior of the theoretical bound. }}
    \label{fig:3d_double_1}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_3d_double32.pdf}
     %   \caption{$\beta = 64$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_3d_double48.pdf}
%\caption{$\beta = 60$}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_rel_3d_double64.pdf}
%\caption{$\beta = 56$}
\end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_3d_double32.pdf}
   %     \caption{$\beta= 64$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_3d_double48.pdf}
%\caption{$\beta = 60$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/precision_norm_3d_double64.pdf}
%\caption{$\beta = 56$}
    \end{subfigure}
 \caption{3-d Example with double precision:  componentwise relative error (top) and block relative error (bottom) with respect to the difference in exponents ($e_{max}-e_{min}$) for $\beta = \{32,48,64\} ${. The blue band represents the sampled maximum and minimum of the error and the red line depicts the theoretical bound. }}
    \label{fig:3d_double_4}
\end{figure}


%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Real-world Viscosity example in double precision 
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Real-World Example}
\label{ex:RealWorld}
%So far, the error analysis as been conducted for a single block of
%generated data.
For this example, we compress data from a real-world three-dimensional
viscosity and density field from 
a Rayleigh-Taylor instability simulation produced by Miranda
\cite{viscosity}. For the viscosity field, the average exponent range over all blocks is
approximately 7.32. This data set is a highly variable example, as the viscosity
values are signed and have a high dynamic range.  The density field has a much smaller dynamic range than the viscosity field. That means the density field is a more compressible data set for ZFP. For both fields, the same value of
$\beta$ was used across all blocks during 
compression to simplify the visualization of the results. In Figure
\ref{fig:viscosity} and \ref{fig:density}, the block relative error is plotted after the data
has been compressed and decompressed (blue) as a function of
$\beta$. The theoretical bound is plotted in red.  Again, we conclude
that the theoretical bound completely bounds the true error for both examples. As for the compression ratio, since the density field has a smaller dynamic range, there is a substantial increase in the compression ratio for every bit plane removed, especially compared to the viscosity field. It can be concluded, that for some error tolerance, ZFP compresses at a higher ratio for data that is ``smooth," i.e., the exponent range for each block is small. 

\begin{figure}
    \centering
                    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/viscocity.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/viscocity_error_norm.pdf}
        \end{subfigure}
             \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/viscocity_error_normratio.pdf}
        \end{subfigure}
        
                
        
        
           \caption{3-d viscosity field example with double precision. On the left is a 3-d rendering of the viscosity field. In the middle is the maximum block relative error as a function of the precision parameter $\beta$. The blue line is the error from ZFP compression and decompression with fixed $\beta$ and the red line depicts the theoretical bound. On the right is the compression ratio as a function of $\beta$.  }
                              \label{fig:viscosity}

\end{figure}
  
  
\begin{figure}
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/miranda-density.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/density_error_norm.pdf}
        \end{subfigure}
             \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/density_error_normratio.pdf}
        \end{subfigure}
            \caption{3-d density field example with double precision. On the left is a 3-d rendering of the density field. In the middle is the maximum block relative error as a function of the precision parameter $\beta$. The blue line is the error from ZFP compression and decompression with fixed $\beta$ and the red line depicts the theoretical bound. On the right is the compression ratio as a function of $\beta$.  }
                              \label{fig:density}

\end{figure}

%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Heat Example with various precisons
%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{2-d Diffusion Example}
%\label{sec:heat}
%In the next example, we wish to test the bounds of the propagation of
%the additional error introduced by ZFP in an iterative method, as
%derived in Proposition~\ref{IterativeProp2}.  
%In the interest of using notation common to the PDE literature, the
%notation we use in this subsection differs from the rest of the paper:
%$x,y$ are the spatial variables, $t$ is the temporal variable, $u$ the
%continuous solution to the heat equation, and ${\bf u}$ is used for
%the uncompressed solution to the discretized diffusion equations.   
%
%The specific PDE we solve, with its initial and boundary conditions, is
%\begin{equation*}
%\begin{array}{rclcrcl}
%\partial_t u(x,y,t)   & = &a\left( \partial_{xx} u(x,y,t)+  \partial_{yy} u(x,y,t)\right ),  && (x,y,t) &\in& [0,1] \times [0,1] \times [0,1], \\
%\end{array}
%\end{equation*}
%\begin{equation*}
%\begin{array}{rclcrcl}
%u(x,y,t) &=& 0 \quad  \forall x,y \in \partial \Omega, \quad   t\in  [0,1],& \text{and} &u(x_{0},y_{0}, t=0) = 1,&&
%\end{array}
%\end{equation*}
%for constant $a$. Using a forward in time and central in space finite
%differences equation is expressed as  
%\[ u_{i,j}^{n+1} = u_{i,j}^n +a \Delta t \left( \frac{u_{i,j+1}^n-2u_{i,j}^n+u_{i,j-1}^n }{\Delta y^2 } +\frac{u_{i+1,j}^n-2u_{i,j}^n+u_{i-1,j}^n}{\Delta x^2 }\right ),  \]  
%for $i,j = 1, ..., 99$, $\Delta x = \Delta y = 1/100$, and Dirichlet boundary conditions enforced by $u_{i,0}^n=u_{0,j}^n = 0\quad \forall i,j$. The initial condition is initialized by setting $u_{49,49} = 1$, an initial heat source in the middle of the block. The finite difference scheme can easily be written as $\bu^{n+1} = A\bu^{n}$,
%where $\bu^{n} = [ u_{i,j}^n ]^{{T}}$ with Lipschitz
%constant $L = \|A\|_\infty = 1$. Let
%$\bv^{n+1} = A({D}_p\tilde{C}_p\bv^{n} )$, where $\bv^{0} = \bu^{0}$.  
%
%In Figure~\ref{fig:heat}, the blue lines depict the error introduced by decompression and
%recompression of the solution at each time step, %block-error,  
%${ \| \bv^{n+1} - \bu^{n+1} \|_{\infty} /\|\bu^{n+1} \|_{\infty}}$.  The
%green line represents the total numerical error, which, for the mesh
%resolutions chosen, is dominated by truncation error:
%${ \| \hat{\bu}^{n+1}- \bu^{n+1}  \|_{\infty}/\|\bu^{n+1} \|_{\infty}}$, where $$\hat{\bu}(x,t)
%=\Delta x^2 \frac{ e^{-\Delta x^2((x - x_0)^2 + (y - y_0)^2) / (4 \pi t)}}{ 4 \pi a t } $$ is the exact solution 
%evaluated in double precision. The red lines represents the theoretical
%bound from Theorem~\ref{IterativeProp2},
%\begin{equation*}
%\frac{\sum_{j = 0}^{n} L^{n-j+1} K_{\beta_j} \|\bu^{j}\|_{\infty}}{\|\bu^{n+1} \|_{\infty}},
%\end{equation*}
%where $\beta_j = \{ 64,54,44,34 \}$ is constant for each experiment
%presented.    
%
%For all $\beta_j$, the theoretical prediction bounds the sampled relative
%error. As $\beta_j$ decreases, the relative sampled error from lossy
%compression and the theoretical bound both increase slowly during the
%time-stepping iterations and trend in a similar way.  The truncation-dominated
%numerical error is well above the sampled error, which means that the
%error introduced by ZFP, for all $\beta_j$,
%is dominated by the the error caused by discretization. We can conclude,
%that even though ZFP is introducing error into the numerical simulation,
%the method remains stable, as the theorem predicts.
%
%\begin{figure}
%    \centering
%        \begin{subfigure}[b]{0.35\textwidth}
%        \includegraphics[width=\textwidth]{figures/heat_error64.pdf}
%        \caption{$\beta= 64$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.35\textwidth}
%        \includegraphics[width=\textwidth]{figures/heat_error54.pdf}
%        \caption{$\beta= 54$}
%    \end{subfigure}
%    
%    \begin{subfigure}[b]{0.35\textwidth}
%        \includegraphics[width=\textwidth]{figures/heat_error44.pdf}
%\caption{$\beta = 44$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.35\textwidth}
%        \includegraphics[width=\textwidth]{figures/heat_error34.pdf}
%\caption{$\beta = 34$}
%    \end{subfigure}
%    \caption{2-d Diffusion Example{: The blue line represents ZFP
%        error, the green line represents the truncation error, and the red
%        line represents the theoretical bound.} } 
%    \label{fig:heat}
%\end{figure}
%
%
%
%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Lax-Wendroff Example with various precisons
%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{1D Advection Example}
%\label{sec:laxwend}
%
%%In the next example, we wish to test the bounds of the propagation of
%%the additional error introduced by ZFP in an iterative method, as
%%derived in Proposition~\ref{IterativeProp2}. 
%In our final example, we have selected the hyperbolic advection
%equation in 1D, as any error generated by compression will be less damped
%than in a system that involves explicit diffusion.    
%Classical discretizions of this PDE result in a small amount of
%artificial dissipation, and we use the Lax-Wendroff scheme, which contains a
%small amount of implicit dissipation that helps to stabilize the
%method. The 
%leading-order truncation error is actually dispersive.  
%Solving a discrete system with weak diffusion results in error that may
%grow over time like the worst-case theoretical bound of the iterative
%method expressed in (\ref{IterativeProp2}) does, although the rate of
%growth is typically nowhere near the worst case for reasonably smooth
%initial data.
%Using similar notation as the previous example, let 
%$x$ be the spatial variable, $t$ the temporal variable, $u$ the
%continuous solution to the advection equation, and ${\bf u}$ the
%uncompressed solution to the discretized advection equations.    
%
%The specific PDE we solve, with its initial and boundary conditions, is
%\begin{equation*}
%\begin{array}{rclcrcl}
%\partial_t u(x,t) +a \partial_x u(x,t)  & = & 0,  && (x,t) &\in& [0,1] \times [0,1], \\
%u(x=0,t) & = & u(x=1,t), && t & \in&  [0,1], \\ 
%u(x, t=0) & = & f(x), && x &\in& [0,1],
%\end{array}
%\end{equation*}
%for constant $a$.  
%The general analytic solution is $u(x,t) = f(x - at)$, representing a
%wave moving in the positive $x$-direction when $a>0$.  The Lax-Wendroff
%scheme is a second-order accurate finite differencing method, expressed
%as   
%\[ u_i^{n+1} = u_i^n -a\frac{\Delta t}{2\Delta x } \left [ u_{i+1}^n - u_{i-1}^n \right ] +a^2 \frac{\Delta t^2}{2\Delta x^2 } \left [ u_{i+1}^n -2u_i^n+ u_{i-1}^n \right ],  \]  
%for $i = 1, ..., 100$ and periodicity enforced by $u^n_0:=u^n_{100}$ and
%$u^n_{101} := u^n_1$.   
%
%Let $a =1$, $\Delta x$ = 1/100, $\Delta t = 1/1000$, such that the CFL
%number is $\sigma=a\Delta t /\Delta x = 1/10$. 
%The Lax-Wendroff scheme can again be written as $\bu^{n+1} = A\bu^{n}$,
%where $\bu^{n} = [ u_1^n, \cdots, u_{100}^n]^{{T}}$ with Lipschitz
%constant $L = \|A\|_\infty=|1-\sigma^2|+|\sigma|\approx 1.09 $. We note
%that, for any $0<\sigma<1$, $L>1$, so the bound of Theorem~\ref{IterativeProp2} will
%grow exponentially with each time step (iteration).  Nevertheless, we
%investigate this type of problem to demonstrate that the theoretical
%bound is overly conservative.
%
%Define $\bv^{n+1} =
%A(\tilde{D}_p\tilde{C}_p\bv^{n} )$, where $\bv^{0} = \bu^{0}$.
%For initial condition $u(x,0) = \sin(2\pi x)$, the blue lines in
%Figure~\ref{fig:laxwend} depict the error introduced by decompression and
%recompression of the solution at each time step, %block-error,  
%${ \| \bv^{n+1} - \bu^{n+1} \|_{\infty} }/ \|\bu^{n+1} \|_{\infty}$.
%The green lines represent the truncation-dominated total numerical error,
%${ \| \bu^{n+1} -  \hat{\bu}^{n+1} \|_{\infty}}/\|\bu^{n+1} \|_{\infty}$, where $\hat{\bu}(x,t)
%=\sin(2\pi(x+at))$ is the exact solution 
%evaluated in double precision. The red lines represent the theoretical
%bound from Theorem~\ref{IterativeProp2},
%\begin{equation*}
%\frac{\sum_{j = 0}^{n} L^{n-j+1} K_{\beta_j} \|\bu^{j}\|_{\infty}}{\|\bu^{n+1} \|_{\infty}},
%\end{equation*}
%where $\beta_j = \{ 56,48,40 \}$ is constant for each experiment
%presented.    
%For all $\beta_j$, the compression error is less than the truncation error
%caused by discretization. Even though the bound (red) from
%Theorem~\ref{IterativeProp2} grows exponentially, the error from
%compression empirically grows at roughly the same rate as the truncation
%error. Clearly, more work is needed to develop a tighter bound for
%Theorem~\ref{IterativeProp2} for hyperbolic problems.
%
%\begin{figure}
%    \centering
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/lax-wend56.pdf}
%        \caption{$\beta= 56$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/lax-wend48.pdf}
%\caption{$\beta = 48$}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\textwidth}
%        \includegraphics[width=\textwidth]{figures/lax-wend40.pdf}
%\caption{$\beta = 40$}
%    \end{subfigure}
%    \caption{1-d Lax-Wendroff Example{: The blue line represents ZFP
%        error, the green line represents the truncation error, and the red
%        line represents the theoretical bound.} } 
%    \label{fig:laxwend}
%\end{figure}


==> qdot-error-bound.tex <==
\section{Error Analysis for qdot} \label{sec:qdot-error-bound}

\textcolor{red}{(I am planning on removing this section as I moved the error analysis fit better in the previous section.)} This approximate kernel introduces additional computation costs towards the front end of a standard dot product but has the potential to make up for these additional costs on the back end by computing some products in lower precision and perforating computation of componentwise products that were identified as unnecessary for the tolerable level of approximation. Additionally, the steps added to the front end of the approximate kernel can be split into two stages that can each be done in parallel. The first stage has the potential to be fast since it consists of $n$ \texttt{short int} addition operations of elements in low precision. %(even if the original vectors are in \texttt{quad} precision we can add the exponents as \texttt{short} integers). 
The second stage where the components are binned by exponent values has the potential to use more time and will have to be cleverly executed. Performance gains will be highly dependent on the input vectors. Higher gains would be observed in vectors where more components can be computed in lower precision or avoided.
%There are potential issues with this approach that will need to be considered and addressed during the analysis phase to determine if this approach is valid. For example, in cases where the terms in the dot product have mixed signs the analysis will be more complicated. Fortunately, computing the norm of a vector is a popular operation in scientific computing which would be an application of this approach where the terms in the dot product are all positive. 
A toy example illustrating \textbf{qdot} can be found in Appendix~\ref{sec:appendixb}.

%At the moment, I am not completely sure that this will work in general. It will clearly work for special cases but I imagine there might be instances where the set of discarded components ends up contributing some information required to achieve the desired accuracy. I will attempt to construct some examples where things go poorly to see how we could correct for them. 

While Algorithm~\ref{alg:q-dot} makes use of exact binning to determine the precision of each component, there are other strategies for selecting bins that could be used instead. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\textbf{Acceptable Bin Precision for CPMS}: We now provide a remark on using the CPMS approach from \cite{cojean2020customized} for determining precision bins. Since this is only included to convey the basic idea, it is not provided in completely general terms. In particular, we provide ranges identifying the segmentation assigned to a bin based on its bin score.

Use the following rules to identify the level of segmentation at which dot product for each bin should be computed. These rules assume that $\bm{x}, \bm{y} \in \mathbb{R}^n$ are stored as 64-bit 4-segment CPMS arrays.  Note that we also provide a \texttt{half} precision bin which is used instead of the 1-segment CPMS. This is due to the fact that the 1-segment CPMS from \cite{cojean2020customized} only has 4 mantissa bits yielding an insignificant range for the bin score to fall within.
\[ 
\text{Precision} (B_{\ell_k,u_k}(\bm{x}, \bm{y}) ) = \left\{
   \begin{array}{lcl}
      \texttt{4-Segment} &:& \beta_k \geq 36 \\
      \texttt{3-Segment} &:& \beta_k \in [20, 36) \\
      \texttt{2-Segment} &:& \beta_k \in [10, 20) \\
      \texttt{Half} &:& \beta_k \in [0, 10) \\
      \texttt{Perforate} &:& \beta_k < 0
   \end{array}
   \right.,
\]
where \texttt{Perforate} indicates that it is not necessary to compute dot product for bin $k$.

The \texttt{4-Segment} is the same as \texttt{double} precision while the \texttt{2-Segment} is very similar to \texttt{single} precision (has 3 fewer mantissa bits and 3 more exponent bits than \texttt{single}). \texttt{Half} is used instead of the \texttt{1-Segment} representation as \texttt{1-Segment} would only be used for $\beta_k \in [0,4)$ which is less likely to happen. Additionally, as we would like to take advantage of Tensor Cores on the GPU, we want to make sure that we compute dot products for values in \texttt{Half} precision.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
